Towards Robust Drone Vision in the Wild

The past few years have witnessed the burst of drone-based applications where computer vision plays an essential role. However, most public drone-based vision datasets focus on detection and tracking. On the other hand, the performance of most existing image super-resolution methods is sensitive to the dataset, specifically, the degradation model between high-resolution and low-resolution images. In this thesis, we propose the first image super-resolution dataset for drone vision. Image pairs are captured by two cameras on the drone with different focal lengths. We collect data at different altitudes and then propose pre-processing steps to align image pairs. Extensive empirical studies show domain gaps exist among images captured at different altitudes. Meanwhile, the performance of pretrained image super-resolution networks also suffers a drop on our dataset and varies among altitudes. Finally, we propose two methods to build a robust image super-resolution network at different altitudes. The first feeds altitude information into the network through altitude-aware layers. The second uses one-shot learning to quickly adapt the super-resolution model to unknown altitudes. Our results reveal that the proposed methods can efficiently improve the performance of super-resolution networks at varying altitudes.

==> head/acknowledgements.tex <==
% \chapter*{Acknowledgements}
% ~\newline~\newline~
% \markboth{Acknowledgements}{Acknowledgements}
% \addcontentsline{toc}{chapter}{Acknowledgements}
% % put your text here
% In the beginning, I would like to give thanks to my supervisor, Dr. Majed El Helou, for his support and help. He immensely cared about my project and always gave me some helpful advice. I am also grateful for Baran Ozaydin and Vidit Vidit. They gave me many suggestions when I met a problem. In addition, I am thankful to my advisor Prof. Süsstrunk Sabine for her support.

% I must also thank my family, especially my parents, Ying Lin and Defeng Wu. They funded my studies here at the EPFL and gave me this valuable opportunity to study aboard.

% % I would also like to thank Koheron company for their help at the beginning of this project.

% \bigskip
 
% \noindent\textit{Lausanne, 1 July 2022}
% \hfill Xiaoyu Lin


==> head/dedication.tex <==
\cleardoublepage
\thispagestyle{empty}


\vspace*{3cm}

\begin{raggedleft}
    	Wings are a constraint that makes \\
	it possible to fly.\\
     --- Robert Bringhurst\\
\end{raggedleft}

\vspace{4cm}

\begin{center}
    To my parents\dots
\end{center}




==> tail/cv/cv.tex <==
\cleardoublepage
\thispagestyle{empty}
\phantomsection
\addcontentsline{toc}{chapter}{Curriculum Vitae}

% NOTE: If you want to make your life hard and write your CV in Latex keep the following lines as they are. If you desire to upload a pre-made PDF CV please uncomment the next line and comment the line just after it.
% \includepdf[pagecommand=\thispagestyle{addpagenumbersforpdfimports},pages=-]{tail/cv/cv.pdf} % To upload a PDF CV directly
\subfile{tail/cv/cv_main.tex} % To do cv with LaTeX
